When Prompt Engineering Meets Software Engineering: CNL-P as Natural and Robust "APIs'' for Human-AI Interaction

With the growing capabilities of large language models (LLMs), they are increasingly applied in areas like intelligent customer service, code generation, and knowledge management. Natural language (NL) prompts act as the ``APIs'' for human-LLM interaction. To improve prompt quality, best practices for prompt engineering (PE) have been developed, including writing guidelines and templates. Building on this, we propose Controlled NL for Prompt (CNL-P), which not only incorporates PE best practices but also draws on key principles from software engineering (SE). CNL-P introduces precise grammar structures and strict semantic norms, further eliminating NL's ambiguity, allowing for a declarative but structured and accurate expression of user intent. This helps LLMs better interpret and execute the prompts, leading to more consistent and higher-quality outputs. We also introduce an NL2CNL-P conversion tool based on LLMs, enabling users to write prompts in NL, which are then transformed into CNL-P format, thus lowering the learning curve of CNL-P. In particular, we develop a linting tool that checks CNL-P prompts for syntactic and semantic accuracy, applying static analysis techniques to NL for the first time. Extensive experiments demonstrate that CNL-P enhances the quality of LLM responses through the novel and organic synergy of PE and SE. We believe that CNL-P can bridge the gap between emerging PE and traditional SE, laying the foundation for a new programming paradigm centered around NL.

==> sections/conclusions.tex <==
\section{Conclusions}

While LLMs provide significant flexibility and capability in processing natural language, certain roles of CNLs—especially at the domain-specific and macro levels—remain relevant for ensuring structured, precise,
and unambiguous communication in software development and other critical applications.

==> sections/design_philosophy.tex <==
\section{Design Philosophy for CNL for Human-AI Interaction}

CNL design dimensions from SE: Macro-level - SE principles; Micro-level - API designs, PL constructs

Inspirations from existing CNLs: Representative CNLs from different application domains and their supports for CNL design dimensions

Different Controlled Natural Languages (CNLs) work at different levels of information granularity in software development is accurate and insightful. See the commented-out text below.

Inspirations from PE: PE patterns for micro-level CNL construct design

\begin{comment}
Here's an analysis and critique:
Analysis:
Micro-Level CNLs:

ACE (Attempto Controlled English) and CLCE (Common Logic Controlled English):

These CNLs are suited for expressing precise, low-level rules, requirements, or constraints. They help formalize individual requirements, logical conditions, or domain rules, ensuring
unambiguous interpretation.

Example: Formalizing "Every user must have a unique ID" using logical structures suitable for automated reasoning or rule-based validation.

Macro-Level CNLs:

Use Case Descriptions and Gherkin:
These languages operate at a higher level, focusing on broader scenarios, user interactions, and acceptance criteria. They provide a structured way to capture functional requirements and
scenarios.

Example: Gherkin's "Given-When-Then" format describes user stories and acceptance tests to validate system behavior in different scenarios.

Critique:

Complementary Roles:

Your understanding correctly identifies that different CNLs cater to different levels of software abstraction. Micro-level CNLs like ACE and CLCE are ideal for specifying low-level rules and
constraints, whereas macro-level CNLs like Gherkin and Use Case Descriptions provide a broader view of user interactions and system functionality.

Strengths and Limitations:

While ACE and CLCE are powerful for formalizing specific rules, they may be too granular for capturing overall system behavior or user experience. Conversely, Gherkin and 
Use Case
Descriptions provide a holistic overview but lack the formal rigor for specifying detailed constraints or logic.

Integration Potential:

These CNLs can complement each other within a development process. For example, use Gherkin for high-level scenario descriptions and ACE or CLCE for detailing the specific rules or business
logic within those scenarios.

Flexibility and Scope:

This distinction also highlights that CNLs are versatile tools adaptable to different development needs and stages. However, relying solely on one type may not cover all necessary granularities or
development perspectives.

Your analysis is correct in recognizing that different CNLs serve various levels of information granularity in software development, emphasizing their complementary roles in capturing both high-level scenarios and low-level requirements. The challenge lies in effectively integrating these CNLs to ensure comprehensive software specification and development.
\end{comment}

==> sections/discussion.tex <==
\section{Discussion}

SPL as executable requirements: alternative flows+exception (inspired by use case), SPL examples and scenarios (inspired by Gherkin user stories) - NL BDD, Requirement Inspection, Doctest for input-output pairs, Hypothesis for property based testing. See the commented-out text below.

\begin{comment}
 SPL examples and scenarios  Benefits

Self-Documenting:

This syntax makes the function's intended use and potential misuse clear directly within the function definition, acting as a form of inline documentation.

Testing and Validation:

The examples can be used for automated testing, where the correct examples are verified for expected output, and the incorrect examples are tested to ensure that the function raises the correct exceptions.

Educational Value:

This feature could be particularly useful in educational contexts, where it’s important to teach both how to use functions correctly and what common mistakes to avoid.

Python Doctest, Hypothesis (property-based testing)
\end{comment}

Agent guardrails: separation of concerns, guardrail definition, application and exception handling

SPL2Code: Full stack SPL compiler, separation of what and how, differentiate from NL-PL tight coupling.

SPL agent as a new form of software integrated with broader SE activities (generative UI, technical documentation - reStructuredText)

\begin{comment}

1. cnl有机融合pe技巧和se成熟技术（尤其是re use case and gherkin user stories）

2. 有效分离agent需求和实现：非计算机人员只需关注并可以直观描述需求what，spl compiler严谨地编译成可执行程序how（包括利用现有llm编程框架比如langchain, sk, dspy,  以及编程语言扩展比如guidance, appl）

3. 结构语法和清晰语义同时降低人和ai表述，理解，执行执行自然语言指令认知门槛

4. 严谨可控的nl2code编译流程，支持语法语义错误的早发现早修复，可支持多层次编译优化（multiagent graph，agent workflow，and agent elements and commands，类比系统级，单元级，statement级）

5. 支持自然语言BDD，变炼金术式trial and error agent开发为系统化的agent迭代优化。通过模拟agent行为，无需agent实现，做到需求和设计问题早发现早修复，并保证agent可靠演化。

6. 为generative ui提供精准的agent输入输出和行为定义，支持生成non-chatbot-style human ai interfaces。

7. All in SPL natively, no awkward nl-code conversion, 母子agent同质

\end{comment}

\begin{comment}
记录三个可能讨论点：

1. spl native表示agent所以方面解决prompt+code混搭来回转换的痛点

2. cnl+compiler设计分离what and how，有效衔接agent/prompt技巧和开发llm app的各种pl/se技术

3. spl天然作为agent文档，无缝融入已有软件工具链
\end{comment}

Domain-Specific SPL (see the commented-out text below):  
... applications
where absolute precision, consistency, and traceability are required (e.g., automated theorem proving, regulatory compliance)
... handling specialized data and requests, LLMs, while capable of processing various domains,
might not always achieve the level of domain-specific rigor and reliability needed without a controlled vocabulary.

\begin{comment}
Your thoughts present a nuanced perspective on the evolving role of CNLs with the advent of LLMs: 

1. Diminished Need for Formalized CNLs: LLMs can handle complex natural language inputs with high precision, reducing the necessity for highly formalized CNLs like ACE and CLCE, except where strict,
deterministic interpretations are crucial (e.g., legal or regulatory contexts).

2. Domain-Specific CNLs Remain Relevant in Specific Applications: Domain-specific CNLs could still be necessary for handling specialized data and requests, but they are less needed for general-purpose
applications where LLMs can adapt flexibly.

3. Macro-Level CNLs for System Description: Macro-level CNLs will likely continue to be relevant for describing overall system behaviors, structures, and scenarios. Even if not in their current forms (like
Gherkin), the need for structured descriptions of high-level behavior remains.

Formalized CNLs: Your point aligns with the observation that LLMs can handle a broad range of complex text, diminishing the need for formalized CNLs in general applications. However, for applications
where absolute precision, consistency, and traceability are required (e.g., automated theorem proving, regulatory compliance), formalized CNLs may still play a role that LLMs cannot fully replace due to their
non-deterministic nature.

Domain-Specific CNLs: I agree that domain-specific CNLs may still be necessary when high accuracy and specific domain knowledge are essential. LLMs, while capable of processing various domains,
might not always achieve the level of domain-specific rigor and reliability needed without a controlled vocabulary.

Macro-Level CNLs: Your argument that macro-level CNLs will continue to be relevant for describing high-level system structures and behaviors is valid. LLMs can assist in generating such descriptions, but
a structured language or framework may still be required to ensure clarity, consistency, and effective communication among different stakeholders (developers, managers, clients, etc.).

\end{comment}


==> sections/experiments.tex <==
\section{Experiments}

RQ1: SPL-guided agent design and optimization

RQ2: Response accuracy, response predictability, robustness to NL variations

RQ3: NL static analysis

==> sections/introduction.tex <==
\section{Introduction}
In the context of AI, particularly in models like GPT-4, a "prompt" refers to the input that guides the model’s output. Prompt engineering involves crafting these inputs in a way that guides the model to produce desired outputs. It can involve specifying parameters, providing examples, or framing instructions in a certain way. 

Considering foundation models like GPT-4 as an "AI operating system," it is conceivable to say that "prompt is a new form of API for the AI operating system." This analogy can work well in explaining the role of prompts in interacting with such large-scale AI models to a varied audience. 

Underlying rationale is as follows:

Interfacing with the AI: Prompts serve as a mechanism through which users can interact with and instruct the AI model, similar to how APIs (Application Programming Interfaces) allow different software applications to communicate and issue commands to each other. 

Guiding Behavior: Prompts guide the outputs and behaviors of the AI model in a manner akin to APIs, which define possible interactions with software applications. 

Accessibility: Just like APIs enable developers to leverage pre-built functionalities of a software application, prompts enable users to access and utilize the capabilities of AI models without needing to understand or manipulate the underlying mechanisms. 

Nuances to Consider:

Expressive Limit: While APIs in traditional software can often handle complex, chained, and varied requests, prompts might
have limitations in expressing complexity and handling varied tasks in a single interaction.

State Management: Traditional APIs often have mechanisms for managing state and handling persistent data across
interactions, while prompts, especially in stateless models like GPT-4, do not maintain state or memory across interactions.

Response Predictability: APIs typically have defined and predictable responses based on their documentation, whereas
responses to prompts in AI models like GPT-4 might have some level of variability and unpredictability.

To address these nuances, limitations of existing approaches:

PL + abstraction and templates (LangChain, Semantic Kernel, DSPy) or language extensions (Guidance, LMQL, SGLang, APPL): improve all three nuances, but incur new problems (prompt-code tight coupling, complex NL-PL conversion and wrapping see more comments below)

First principle: why must code in PL? can it be NL programming?

NL + style guides or patterns: may improve response predictability, but nothing else;
micro-level incremental upgrade, no macro-level SE ingredients if regarding prompts as a new form of software

Our solution: design a CNL and supporting agents
First principle: CNL and its benefits

\begin{comment}
其中最核心的痛点是“逼迫”模型按照特定的格式进行输出（比如 JSON），需要写复杂的解析器（Parser）去捕捉修复输出的很多边缘情况（Edge Case）

1. Prompt 与代码⾼度耦合。⼀个好的 Prompt 需要⻓时间的调试和优化才能达到预期效果，但与此同时，实现 Prompt 的代码通常很简单，只是起到⼀个逻辑串联的作⽤。这导致 Prompt ⼯程师和开发者的⼯作⽆法有效分离，整个开发过程效率低下。

2、对⾮技术⼈员完全不友好。Prompt 的调试实际上需要语⾔和领域专家进⾏语义上的迭代优化。但是传统的代码开发⽅式将 Prompt 封装在代码逻辑中，使得语⾔专家和⾮技术⼈员⽆法参与 Prompt 开发和优化过程，⽆法发挥他们的专⻓。

这样的开发⽅式导致 Prompt ⼯程很难落地。我们需要实现 Prompt 与代码的解耦，以更好地发挥语⾔专家和⾮技术专家的作⽤，让 Prompt ⼯程像其他软件⼯程流程⼀样实现⻆⾊分⼯、协作开发。
\end{comment}

==== First principles analysis ====

1. Identifying and Defining the First Principles

Fundamental Nature of Coding: Recognize that coding, involving writing instructions in a programming language, is the core method of creating software.

Software Engineering Principles: Acknowledge established principles like modularity, abstraction, encapsulation, and maintainability as foundational to good software design and development.

2. Deconstructing the Problem

Complexity and Accessibility in Coding: Traditional coding can be complex and inaccessible to those without specialized training, limiting wider participation in software development.

Evolving Role of AI in Software Development: AI, especially in the form of generative AI, is changing how coding is done, potentially automating or simplifying aspects of the coding process.

Need for a More Intuitive Approach: There's a growing need for more intuitive and accessible ways to program, which can democratize software development and make it more efficient.

3. Reconstructing the Problem (at the end of intro to introduce CNL?)

Development of CNL for Software Engineering: Propose the creation of a Controlled Natural Language as an alternative approach to traditional coding. This CNL would allow users to write instructions in a format closer to natural language, making software development more accessible.

Incorporation of AI and Semantic Understanding: Integrate AI capabilities to interpret CNL and translate it into executable code. This involves using AI not just as a tool for automation but as an interpreter between human linguistic input and machine-readable code.

Designing CNL with First Principles in Mind: Construct the CNL in a way that adheres to software engineering first principles. This includes ensuring that the CNL supports modularity, abstraction, and other key principles, while also being easy to use and understand.

Special Keywords and Structured Approach: Introduce special keywords (like @persona, @task) in CNL to provide structure and clarity, ensuring that the language remains both user-friendly and precise enough for software development tasks.

In summary, by applying first principles thinking, the discussion moves from recognizing the fundamental role of coding in software engineering to identifying its limitations in terms of accessibility and efficiency. This leads to the innovative idea of developing a CNL, which is reconstructed to align with core software engineering principles while leveraging AI to bridge the gap between natural language and traditional coding.

==> sections/relatedwork.tex <==
\section{Related Work}

AI4SE: adopt AI to enhance SE practices ... 
"NL-augmented coding" is a concise and descriptive term that captures the essence of what you're trying to convey. "NL" stands for
Natural Language, which makes it clear that the coding is enhanced or augmented by the integration of natural language
capabilities. The term "augmented" suggests an enhancement or extension rather than a replacement, which aligns with your
description of the setup where code serves as the primary mechanism with natural language as an additive layer. Overall, it's a term
that could effectively describe a programming paradigm that incorporates both coded and natural language elements.

SE4AI: on one hand, apply SE principles to transform PE into a new form of SE; on the other hand, the synergy of SE and PE reshapes existing SE practices

Empirical studies: 
Manually developed pseudo-code prompts and empirically demonstrated their effects.
- Language Models of Code are Few-Shot Commonsense Learners
- Prompting with Pseudo-Code Instructions

Pesudo-code prompt: ProgPrompt; THINK-EXECUTE Language Models as Compilers

Pesudo-langs: see the comments
\begin{comment}
SudoLang: the most sophisticated one
•	SudoLang: A Powerful Pseudocode Programming Language for LLMs https://medium.com/javascript-scene/sudolang-a-powerful-pseudocode-programming-language-for-llms-d64d42aa719b (similar to how I use ChatGPT to design and validate SPL)
•	SudoLite: https://www.sjgarstack.org/blog/20231102/introducing-sudolite#about-the-author
•	Better Prompting with Pseudocode – Eric Elliot https://www.youtube.com/watch?v=TADrrG6Fhjk&list=PLQEYbmzcCfpe-3GLDTtwvfF6MpjLVVFZ1&index=8
•	Sudo Lang spec and tutor: https://chatgpt.com/share/1488c408-8430-454f-84b8-fdd1d8f815a2 (Do not actually have compiler and runtime. Prompt LLM to compile and execute the SudoLang prompts.)

Jargon: an LLM-based pseudolanguage for prompt engineering
•	Inspires SudoLang design
•	Jargon interpreter/CLI: https://github.com/jbrukh/gpt-jargon/blob/main/jargon_cli/cli.py (We should support UGAiForge CLI/playground)

LLMScript
•	Introducing LLMScript - A New Ai-Centric Pseudo Programming System https://www.linkedin.com/pulse/introducing-llmscript-new-ai-centric-pseudo-system-reuven-cohen-mcp0c
•	LLMScript spec and runtime: https://gist.github.com/ruvnet/9119f53f50b06628981dfc9d4db0d74c; declarative languages to call Python APIs and tools.

Plang
•	Plang - a new type of programming language https://www.reddit.com/r/programming/comments/1bkynth/plang_a_new_type_of_programming_language/
•	Programming 3.0 – Theory https://www.reddit.com/r/plang/comments/1blpv72/programming_30_theory/ Big claim. Like worker_instruction in SPL.

PseudoLangs
•	Bridging the Gap: How PseudoLangs Enhances Human-AI Collaboration https://promptengineering.org/bridging-the-gap-how-pseudolangs-enhances-human-ai-collaboration/ 
PseudoLangs are synthetic languages created to bridge the gap between human intents and AI abilities. Technical PseudoLangs enable precise outputs while creative ones unlock generative models' imagination through targeted vocabularies and logic.
•	Speak AI Fluently: SudoCode Makes Building Complex AI as Easy as Talking https://promptengineering.org/pseudocode-sudocode-bridging-the-gap-between-humans-and-ai/ 
•	PseudoScript - Structuring Intent for Generative AI https://promptengineering.org/pseudoscript-structuring-intent-for-generative-ai/ At the level of SPL worker instructions.
PseudoScript is a promising new PseudoLang using structured directives to guide AI systems through complex workflows. Its script-like format bridges accessibility and technical precision, making AI creativity more reliable for goals like writing content or developing software.
\end{comment}

NL2Code: PAL- PROGRAM-AIDED LANGUAGE MODELS, Chain of Code Li FeiFei, CodeAct

PL extensions: Guidance, LMQL, SGLang, APPL, MindsDB

NL2DSL2Code: Microsoft natural language commanding via program synthesis; PromptRPA (NL2UIOpsDSL2UIOps), TableGPT (NL2DataOpsDSL2SQL), ReactGenieDSL (NL2MultiModalDSL2APICalls)

PlanSearch: NL to high-level design plan to code, but high-level design plan is not a CNL; SPL for natural and robust requirement analysis and system design.



==> sections/spl.tex <==
\section{Structured Prompting Language (SPL)}

\subsection{SPL Syntax}

All in SPL: agent context, data, command and workflow

Alignment analysis of SPL syntax and CNL design dimensions

CNL PENS analysis 

\subsection{NL-to-SPL Agent}

Analytic flow inspired by human thinking process: 4 steps; 

As an example of SPL-driven agent design ... 
Agent component design guided by SPL syntax, adhering to fundamental SE principles (separation of concerns, modularity) and best PE practices (persona, constraints, CoT)

Benefits for end-user: Balance user friendly, user's cognitive burden and agent's precision and robustness for agent design

This NL-to-SPL agent can generate more SPL agents ... resolve heterogeneous NL-PL problem in PL-extensions based solutions

\subsection{SPL Linting}

First static analysis technique for NL
